Testing Equality of Medians for Multiple Samples

In this paper, we construct a consistent non-parametric test for testing the equality of population medians for different samples when the observations in each sample are independent and identically distributed. This test can be further used to test the equality of unknown location parameters for different samples. The method discussed in this paper can be extended to any quantile level instead of the median. We present the theoretical results and also demonstrate the performance of this test through simulation studies.

==> custom.tex <==
@article{oliveira2024split,
  title={Split conformal prediction and non-exchangeable data},
  author={Oliveira, Roberto I and Orenstein, Paulo and Ramos, Thiago and Romano, Joao Vitor},
  journal={Journal of Machine Learning Research},
  volume={25},
  number={225},
  pages={1--38},
  year={2024}
}

@book{reiss2012approximate,
  title={Approximate distributions of order statistics: with applications to nonparametric statistics},
  author={Reiss, Rolf-Dieter},
  year={2012},
  publisher={Springer science \& business media}
}

@article{bahadur1966note,
  title={A note on quantiles in large samples},
  author={Bahadur, R Raj},
  journal={The Annals of Mathematical Statistics},
  volume={37},
  number={3},
  pages={577--580},
  year={1966},
  publisher={JSTOR}
}

@article{mcmath1981mean,
  title={Mean value theorems for a matrix valued derivative},
  author={McMath, John S and Sims, SE},
  journal={Linear and Multilinear Algebra},
  volume={9},
  number={4},
  pages={255--261},
  year={1981},
  publisher={Taylor \& Francis}
}

@article{tran1992kernel,
  title={Kernel density estimation for linear processes},
  author={Tran, Lanh Tat},
  journal={Stochastic processes and their applications},
  volume={41},
  number={2},
  pages={281--296},
  year={1992},
  publisher={Elsevier}
}

@article{cox1985testing,
  title={Testing the equality of two normal percentiles},
  author={Cox, TF and Jaber, K},
  journal={Communications in Statistics-Simulation and Computation},
  volume={14},
  number={2},
  pages={345--356},
  year={1985},
  publisher={Taylor \& Francis}
}

@article{albers1984approximate,
  title={An approximate confidence interval for the difference between quantiles in a Bio-Medical problem},
  author={Albers, Willem and L{\"o}hnberg, Peter},
  journal={Statistica Neerlandica},
  volume={38},
  number={1},
  pages={20--22},
  year={1984},
  publisher={Wiley Online Library}
}

@article{rudolfer1985large,
  title={Large sample inference for diagnostic normal limits in Gaussian populations},
  author={Rudolfer, SM and Campbell, MG},
  journal={Communications in Statistics-Theory and Methods},
  volume={14},
  number={8},
  pages={1801--1835},
  year={1985},
  publisher={Taylor \& Francis}
}

@book{huang2001confidence,
  title={Confidence regions for the ratio of percentiles},
  author={Huang, Li-Fei},
  year={2001},
  publisher={The University of Wisconsin-Madison}
}

@inproceedings{marshall1950some,
  title={Some test for comparing percentage points of two arbitrary continuous populations},
  author={Marshall, AW and Walsh, JE},
  booktitle={Proceedings of the International Congress of Mathematicians},
  volume={1},
  pages={1--13},
  year={1950}
}

@article{walsh1954bounded,
  title={Bounded significance level tests for comparing quantiles of two possibly different continuous populations},
  author={Walsh, John E},
  journal={Annals of the Institute of Statistical Mathematics},
  volume={6},
  number={3},
  pages={213--222},
  year={1954},
  publisher={Springer}
}



@article{bristol1990distribution,
  title={Distribution--free confidence intervals for the difference between quantiles},
  author={Bristol, DR},
  journal={Statistica Neerlandica},
  volume={44},
  number={2},
  pages={87--90},
  year={1990},
  publisher={Wiley Online Library}
}

@article{wilcox1995comparing,
  title={Comparing two independent groups via multiple quantiles},
  author={Wilcox, Rand R},
  journal={Journal of the Royal Statistical Society Series D: The Statistician},
  volume={44},
  number={1},
  pages={91--99},
  year={1995},
  publisher={Oxford University Press}
}

@article{wilcox1991testing,
  title={Testing whether independent treatment groups have equal medians},
  author={Wilcox, Rand R},
  journal={Psychometrika},
  volume={56},
  pages={381--395},
  year={1991},
  publisher={Springer}
}

@incollection{johnson2003some,
  title={Some exact and approximate confidence regions for the ratio of percentiles from two different distributions},
  author={Johnson, Richard A and Huang, Li-Fei},
  booktitle={Mathematical and statistical methods in reliability},
  pages={455--468},
  year={2003},
  publisher={World Scientific}
}

@article{hin2012rank,
  title={A Rank Test on Equality of Population Medians},
  author={Hin, Pooi Ah},
  journal={Journal of Science and Technology},
  volume={4},
  number={2},
  year={2012}
}
